Dreamcrafter: Immersive Editing of 3D Radiance Fields Through Flexible, Generative Inputs and Outputs

Authoring 3D scenes is a central task for spatial computing applications. Competing visions for lowering existing barriers are (1) focus on immersive, direct manipulation of 3D content or (2) leverage AI techniques that capture real scenes (3D Radiance Fields such as, NeRFs, 3D Gaussian Splatting) and modify them at a higher level of abstraction, at the cost of high latency. We unify the complementary strengths of these approaches and investigate how to integrate generative AI advances into real-time, immersive 3D Radiance Field editing. We introduce Dreamcrafter, a VR-based 3D scene editing system that: (1) provides a modular architecture to integrate generative AI algorithms; (2) combines different levels of control for creating objects, including natural language and direct manipulation; and (3) introduces proxy representations that support interaction during high-latency operations. We contribute empirical findings on control preferences and discuss how generative AI interfaces beyond text input enhance creativity in scene editing and world building.

==> alt-text.tex <==
Figure 1: \Description[Living Room scene showcasing spatial annotations and pipeline for Dreamcrafter connecting the Unity App to external modules for object generation and editing]{(Left) - Visual 3D VR scene depicting the living room of a house. There are various objects such as a couch, chair, table, etc. spread out across the room, each accompanied by a spatial annotation representing the edit information inputted by the user. The couch has an annotation reading “make it grey”, followed by a generated 2D grey version of the couch displayed above the 3D asset. The chair has the edit instruction “make it retro” along with a retro-styled 2D image above. The table has the instruction “place a table”, and depicts a rendered 3D table on the floor. (Right) - Architecture diagram titled Independent Components for Interacting with and Editing Scenes, containing three components: Unity App, Edit Radiance Fields Objects, and Generate new objects in the scene. Edit Radiance Fields Objects contains the following workflow: Unity app feeds into JSON Edit Instruction, which feeds into Offline Radiance Field Editing Model, feeding into Save Updated Model, then Online Radiance Field Preview, and finally back to Unity App. JSON Edit Instruction also directly feeds into Online Radiance Field Preview. Generate new objects in the scene contains the following workflow: Unity app feeds into JSON Create Instruction, which feeds into Offline 3D Object Generation Model, feeding into Save New Generated Model, feeding into Online 3D Object Generation Preview, and finally back to Unity App. JSON Create Instruction also feeds into Online 3D Object Generation Preview.}
Figure 2: \Description[System module diagram showing external models and broker server.]{Four components: Unity Project, Broker Server, Object Generation, Radiance Field Editing. Unity Project serves as the backbone, feeding into and out of the Broker Server. Broker Server independently communicates with Object Generation and Radiance Field Editing independently. Object Generation contains: Online (Preview) component connecting Text-to-3D (Shap-E) to Stylization (ControlNet), and Offline component containing Image to 3D Model. Radiance Field Editing contains: Online (Preview) component containing Image Editing (Instruct-Pix2Pix), and Offline component combining Radiance Field Editors, Instruct-NeRF2NeRF, and Instruct-GS2GS.}
Figure 3: \Description[User is moving a bench outdoors with VR controllers]{User is holding VR controllers to manipulate the scene, in a simulated outdoor environment. They depict rotations, translations, and scaling of a 3D table bench asset in space.}
Figure 4:\Description[A chair radiance field object is edited]{3D chair asset is placed in living room space, with three visual options for modified chair assets. Instructions hover above to “Select Edit Variant”. Upon selection, a single 2D sample modification image is displayed with the edit instruction prompt. Final image depicts a fully modified 3D asset, in style of instruction and 2D image selected.}
Figure 5: \Description[A lamp object is generated via prompting]{Floating selection platform is placed on the floor in a hotel hallway scene. User prompts to “Make an ornate brass lamp”, and is presented with three 2D image options with instructions to “Select Variant”. User selects a single image option, and thereafter a 3D asset is generated and placed in scene matching the image variant selection.}
Figure 6: \Description[A gingerbread house object is sculpted.]{An untextured 3D asset composed of basic shapes is depicted on the floor in a large indoor 3D space, resembling gingerbread house style. Horizontal menu bar appears with options “Shapes, Prompt, Stylize, Confirm, Cancel”. User prompts “Gingerbread House” and 2D image preview of colored and stylized gingerbread house is displayed above the untextured 3D asset. Finally, the 3D asset adopts a fully textured gingerbread house in the scene.}
Figure 7: \Description[An edited scene of a holiday party.]{The scene depicts a floor of a large indoor space. There are various 3D assets rendered around the environment, including an untextured snowman, a generative platform represented by a disc, a fully textured gingerbread house, and a circular table with chairs behind. The snowman is accompanied by a spatial edit instruction “Snowman” and 2D render of a snowman. The platform has a spatial tag “Make a snowy tree” along with a 2D render image. The gingerbread house is fully rendered and stylized. The table is textured, and has a spatial edit to “make it gold and festive” accompanied by a 2D image depicting the new style to implement.}
Figure 8: \Description[Magic camera and panel in a living room scene]{A living room scene with a blue holographic camera and a panel with a preview of a stylized realistic render from the magic camera of its perspective with the text caption "realistic living room" on the panel.}
Figure 9: \Description[Magic camera outputs showing stylized scenes of a living room, outdoor courtyard, and holiday party.]{Three sets of inputs and outputs for the Magic Camera image re-stylizing system. The top row shows the scene inputs: (Left) A living room scene with a sofa and chairs placed in a 3D scene, (Center) An outdoor deck next to a building with benches, chairs, plants, and a 3D model of a cherry blossom tree and chair. (Right) A holiday party scene composed of tables, chairs, a 3D models of a Christmas tree, a snowman, and a gingerbread house in a building atrium. The bottom row shows the coherent photorealistic outputs: (Left) A realistic living room scene with correct lighting and shadows. (Center) An outdoor deck next to a building with stylistically consistent benches and chairs with plants and a realistic tree. (Right) A stylized version of the same holiday party scene in a photorealistic style with realistic lighting and shading. }
Figure 10: \Description[2D and 3D proxy representations]{(Left) Shows a 2D image plane of a stylized table placed in the scene. (Right) Shows a desk chair 3D model with a label “Make a desk chair” and a 2D image of a stylized chair over it.} 
Table 1: \Description[Participant data from user evaluation for tool usage]{Counts of the levels of control (i.e., Editing, Creating via prompting, Creating via sculpting) participants used for each task in the evaluation.}


==> figures.tex <==
\newcommand{\systemOverview}{
  \begin{figure}[h]
    \centering
    \resizebox{0.9\linewidth}{!}{%
      \includegraphics{images/CHI_FigureServerModules.pdf}
    }
    \label{fig:sysOverview}
    \caption{\textbf{Dreamcrafter system overview.} Modules processing pipeline: The Unity project sends API calls to the broker server to run instructions from specific generation modules and their outputs get sent back to the Unity project. Online modules are run for previewing generations, and offline modules are run after editing is complete.}
    \Description{Four components: Unity Project, Broker Server, Object Generation, Radiance Field Editing. Unity Project serves as the backbone, feeding into and out of the Broker Server. Broker Server independently communicates with Object Generation and Radiance Field Editing independently. Object Generation contains: Online (Preview) component connecting Text-to-3D (Shap-E) to Stylization (ControlNet), and Offline component containing Image to 3D Model. Radiance Field Editing contains: Online (Preview) component containing Image Editing (Instruct-Pix2Pix), and Offline component combining Radiance Field Editors, Instruct-NeRF2NeRF, and Instruct-GS2GS.}
  \end{figure}
}


\newcommand{\moveObjects}{
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/move_obj.png}
\caption{\textbf{Object transformations and direct manipulations:} (Left) Positioning object in the scene (Center) Rotating object. (Right) Scaling object}
\label{fig:moveObjs}
\Description{User is holding VR controllers to manipulate the scene, in a simulated outdoor environment. They depict rotations, translations, and scaling of a 3D table bench asset in space.}
\end{figure}
}

\newcommand{\objectEdit}{
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/obj_edit_v2.png}
\caption{\textbf{Radiance Field Object Editing with preview:} (Left) Edit variants are presented to a user. (Center) Displaying selected edit preview as a spatial annotation. (Right) Fully processed 3D edit replaces the original}
\label{fig:objEdit}
\Description{3D chair asset is placed in living room space, with three visual options for modified chair assets. Instructions hover above to “Select Edit Variant”. Upon selection, a single 2D sample modification image is displayed with the edit instruction prompt. Final image depicts a fully modified 3D asset, in style of instruction and 2D image selected.}
\end{figure}
}

\newcommand{\objectPromptGen}{
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/obj_prompt_generation_v3.jpg}
\caption{\textbf{Object Generation via Prompting:} (Left) Object generation variations from speech input. (Center) Displaying selected generation preview as a spatial annotation. (Right) Fully processed 3D generation in the scene.}
\label{fig:objPromptGen}
\Description{Floating selection platform is placed on the floor in a hotel hallway scene. User prompts to “Make an ornate brass lamp”, and is presented with three 2D image options with instructions to “Select Variant”. User selects a single image option, and thereafter a 3D asset is generated and placed in scene matching the image variant selection.}
\end{figure}
}

\newcommand{\objectSculptGen}{
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/obj_sd_generation_v2.png}
\caption{\textbf{Object Generation via Sculpting:} (Left) Sculpting toolkit to create primitive shape arrangement (Center) Displaying stylized sculpted object preview as a spatial annotation. (Right) Fully processed 3D generation in the scene.}
\label{fig:objSculptGen}
\Description{An untextured 3D asset composed of basic shapes is depicted on the floor in a large indoor 3D space, resembling gingerbread house style. Horizontal menu bar appears with options “Shapes, Prompt, Stylize, Confirm, Cancel”. User prompts “Gingerbread House” and 2D image preview of colored and stylized gingerbread house is displayed above the untextured 3D asset. Finally, the 3D asset adopts a fully textured gingerbread house in the scene.}
\end{figure}
}

\newcommand{\figproxy}{
\begin{figure}[h]
\centering
 \resizebox{0.9\linewidth}{!}{%
      \includegraphics{images/proxy_2d_3d_v2.png}
}
%\includegraphics[width=\linewidth]{images/proxy_2d_3d.png}
\caption{\textbf{3D and 2D Proxy Representations:} (Left) New 3D proxy showing a low fidelity mesh preview (Right) Original 2D proxy representation with image preview}
\label{fig:figproxy}
\Description{(Left) Shows a 2D image plane of a stylized table placed in the scene. (Right) Shows a desk chair 3D model with a label “Make a desk chair” and a 2D image of a stylized chair over it.}
\end{figure}
}

\newcommand{\magicCamFig}{
\begin{figure*}[h]
\centering
 \resizebox{1.0\linewidth}{!}{%
      \includegraphics{images/CHI_dreamcrafter_magic_camera_outputs_v3.pdf}
}
\caption{\textbf{Magic Camera Outputs:} (Top row) Scene inputs from the virtual Unity camera (Bottom row) Stylized image outputs given the prompts: (Left) "realistic apartment living room", (Center) "realistic outdoor patio in university with cherry blossom tree, chairs, benches, plants", (Right) "a holiday party in a hotel atrium, snowman, Christmas, gingerbread house". The image stylization model generates stylistically consistent and coherent photorealistic image outputs from the input scenes of composed radiance fields and 3D models.}
\label{fig:magicCamFig}
\Description{Figure 9: Three sets of inputs and outputs for the Magic Camera image re-stylizing system. The top row shows the scene inputs: (Left) A living room scene with a sofa and chairs placed in a 3D scene, (Center) An outdoor deck next to a building with benches, chairs, plants, and a 3D model of a cherry blossom tree and chair. (Right) A holiday party scene composed of tables, chairs, a 3D models of a Christmas tree, a snowman, and a gingerbread house in a building atrium. The bottom row shows the coherent photorealistic outputs: (Left) A realistic living room scene with correct lighting and shadows. (Center) An outdoor deck next to a building with stylistically consistent benches and chairs with plants and a realistic tree. (Right) A stylized version of the same holiday party scene in a photorealistic style with realistic lighting and shading. }
\end{figure*}
}

\newcommand{\magicCamPanelFig}{
\begin{figure}[h]
\centering
 \resizebox{1.0\linewidth}{!}{%
      \includegraphics{images/magic_camera_tool_panel.png}
}
\caption{\textbf{Magic Camera:} The virtual camera can be repositioned with a panel previewing the stylized output from the Magic Camera with the given text prompt.}
\label{fig:magicCamPanelFig}
\Description{A living room scene with a blue holographic camera and a panel with a preview of a stylized realistic render from the magic camera of its perspective with the text caption "realistic living room" on the panel.}
\end{figure}
}

\newcommand{\spatialAnnotations}{
\begin{figure}[h]
\centering
 \resizebox{1.0\linewidth}{!}{%
      \includegraphics{images/proxy_editing_scene_v2.png}
}
\caption{\textbf{Spatial annotations:} tags and proxy representations are placed over the radiance field objects and generated objects with given instructions and preview generations.}
\label{fig:spatialAnnotations}
\Description{The scene depicts a floor of a large indoor space. There are various 3D assets rendered around the environment, including an untextured snowman, a generative platform represented by a disc, a fully textured gingerbread house, and a circular table with chairs behind. The snowman is accompanied by a spatial edit instruction “Snowman” and 2D render of a snowman. The platform has a spatial tag “Make a snowy tree” along with a 2D render image. The gingerbread house is fully rendered and stylized. The table is textured, and has a spatial edit to “make it gold and festive” accompanied by a 2D image depicting the new style to implement.}
\end{figure}
}



%\newcommand{\objectSculptGen}{
%\begin{figure}[h]
%\centering
%\includegraphics[width=\linewidth]{images/obj_prompt_generation.png}
%\caption{\textbf{Object Generation via Sculpting} (Left) Sculpting toolkit to create primitive shape arrangement (Center) Displaying stylized sculpted object preview as a spatial annotation. (Right) Fully processed 3D generation in the scene.}
%\label{fig:objSculptGen}
%\end{figure}
%}
